Routing Directions: Keeping it Fast and Simple

The problem of providing meaningful routing directions over road networks is of great importance. In many real-life cases, the fastest route may not be the ideal choice for providing directions in written, spoken text, or for an unfamiliar neighborhood, or in cases of emergency. Rather, it is often more preferable to offer "simple" directions that are easy to memorize, explain, understand or follow. However, there exist cases where the simplest route is considerably longer than the fastest. This paper tries to address this issue, by finding near-simplest routes which are as short as possible and near-fastest routes which are as simple as possible. Particularly, we focus on efficiency, and propose novel algorithms, which are theoretically and experimentally shown to be significantly faster than existing approaches.

==> extensions.tex <==
%!TEX root = main.tex

\section{Extensions}




==> fastest.tex <==
%!TEX root = main.tex


\subsection{Simplest Fastest Route}
\label{sec:fastest}




\begin{algorithm}[t]
\small
\SetInd{0.3em}{0.8em}
\SetCommentSty{textsf}
\SetArgSty{textrm}
\DontPrintSemicolon
\SetKw{Break}{break}
\SetKw{Enheap}{enheap}
\SetKw{Deheap}{deheap}
\SetKw{Retrieve}{retrieve}
\SetKw{Mark}{mark}
\SetKw{Update}{update}
\KwIn{road network $G_R$; function $L$; function $C$; source $n_s$; target $n_t$}
\KwOut{length \textit{sfL} and complexity \textit{sfC} of simplest fastest route from $n_s$ to $n_t$}
\SetKwInput{KwVar}{Variables}
\KwVar{minheap $H$ with entries $\<n, r | len, cpl, n_{prev}, r_{prev}\>$, keys $(len, cpl)$, and compare function $<_{SF}$}

\ForEach{$r_i$ that contains $n_s$}{
	$\la{n_s,r_i} \gets \<n_s,r_i | 0, 0, n_{\varnothing}, r_i\>$\;
	\Enheap $\la{n_s,r_i}$ in $H$ \;
}

\While{$H$ not empty}{
    $\<n_x,r_i | len, cpl, n_w, r_h\> \gets$ \Deheap\;
    \Mark $\la{n_x,r_i}$ as \texttt{final} \;

    \lIf{$n_x$ is $n_t$}{
     	\Break\;
    }
    \lElse{
    	\ForEach{edge $(n_x, n_y)$} {
    	    \ForEach{road $r_j$ that contains $n_y$} {
	    		\If{$\la{n_y, r_j}$ does not exist} {
	    			$\la{n_y, r_j} \gets \<n_y, r_j | len + L(n_x,n_y), cpl + C(n_y, r_i, r_j), n_x, r_i\>$\;
	    			\Enheap $\la{n_y, r_j}$
	    		}
	    		\ElseIf{$\la{n_y, r_j}$ is not \texttt{final}}{
	    			$ \<n_y, r_j | len', cpl', n_u, r_h\> \gets \la{n_y, r_j}$ \;
	         		\If{ $(len + L(n_x,n_y), cpl + C(n_y, r_i, r_j)) <_{SF} (len', cpl')$ } {
						$\la{n_y, r_j} \gets \<n_y, r_j | len \!+\! L(n_x,n_y), cpl \! + \! C(n_y, r_i, r_j), n_x, r_i\>$\;
						\Update $\la{n_y, r_j}$
		     		}
	    		}
    		}
    	}

    }
}
\Return $(\textit{sfL}, \textit{sfC}) \gets (len,cpl)$ \;
\caption{SimplestFastest}
\label{algo:sf}
\end{algorithm}




==> simple.tex <==
%!TEX root = main.tex

\section{Fastest Near-Simplest Route}
\label{sec:near-simplest}

\eat{
We next present an algorithm for Problem~2, i.e., for finding the fastest of near-simplest
routes. Similar to that of Section~\ref{sec:near-fastest}, the key idea is to enumerate all routes from
source to target, eliminating in the process routes which are $(1+\epsilon)$ times more complex that
the simplest route, or are longest than the best found so far.


We next detail the ShortestEasy algorithm, whose pseudocode is shown in
Algorithm~\ref{algo:fastestnearsimplest}. Initially, it uses the AllFastestSimplest procedure, derived
from the FastestSimplest algorithm (Section~\ref{sec:simplest}), to retrieve the complexity and
length of all fastest simplest routes starting from each road and reaching the target node $n_t$.
Then, like EasiestShort, it performs a depth-first search, but on the transition graph $G_I$ using
the stack $S$ and eliminating routes according to two criteria.


The first prunes routes based on their complexity. It computes the complexity of the simplest
possible extension of the current route via the examined transition to the target. This complexity is
one more than that of the current route plus the complexity of the simplest route from the current
road to the target. If the computed complexity exceeds the threshold for an near-simplest route,
the current route is abandoned.


The second criterion prunes routes based on their length. It simply checks whether the extension of
the current route along a transition is longer than the best found.


\stitle{Analysis.} The complexities of AllFastestSimplest are the same as those of
FastestSimplest, i.e, $O(|R|\log |E|)$ for time and $O(|R|)$ for space. Let $C$ denote the
complexity of the fastest simplest route, and $k'$ be the number of possible near-simplest routes from
source to target. At any time the stack of FastestNearSimplest corresponds to a subpath of some near-simplest
route, which may involve at most $(1+\epsilon)C$ edges (but not more than $(1+\epsilon)|R|$).
Therefore, the time complexity is $O(|V|\log|E| + k'(1+\epsilon)C)$, and the space complexity is
$O(|V| + (1+\epsilon)C)$.
}




\eat{

\begin{algorithm}[t]
\small
\LinesNotNumbered
\SetInd{0.3em}{0.8em}
\SetCommentSty{textsf}
\SetArgSty{textrm}
\DontPrintSemicolon
\SetKw{Continue}{continue}
\SetKw{Break}{break}
\SetKw{Find}{find}
\SetKw{Push}{push}
\SetKw{Pop}{pop}
\SetKw{ReadTop}{top}
\SetKw{MyAnd}{and}
\SetKw{Mark}{mark}
\KwIn{road network $G_R$; mapping $C$; source $n_s$; target $n_t$; value $\epsilon$}
\KwOut{length \textit{fnsL} and complexity \textit{fnsC} of fastest near-simplest route from $n_s$ to $n_t$}
\SetKwInput{KwVar}{Variables}
\KwVar{stack $S$ with entries $(n | len, cpl, n_{prev})$}


$(\textit{sfL}[\,],\textit{sfC}[\,]) \gets \mathrm{AllSimplestFastest}(G_R,C,n_t)$ \;
$(\textit{fsL}[\,],\textit{fsC}[\,]) \gets \mathrm{AllFastestSimplest}(G_R,C,n_t)$ \;

\nlset{3}\If{ $\textit{sfC}[n_s] \leq (1+\epsilon)\cdot \textit{fsC}[n_s]$} {
     \nlset{4}\Return $(\textit{fnsL}, \textit{fnsC}) \gets (\textit{sfL}[n_s], \textit{sfC}[n_s])$\;
} 

\nlset{5}$(\textit{fnsL}^+, \textit{fnsC}^+) \gets (\textit{fsL}[n_s], \textit{fsC}[n_s])$ \;

\Push $(n_s | 0, 0, n_{\varnothing})$ \;

\While{$S$ not empty}{
     $(n_x | len, cpl, n_w) \gets $ \ReadTop \;
     
     \If{$n_x$ not \texttt{in\_route} }
     {
          \nlset{10}\lIf{ $len > \textit{fnsL}^+$ } {
               \Pop\;
          }
          \ElseIf{$n_x$ is $n_t$}{
               \nlset{12}$(\textit{fnsL}^+, \textit{fnsC}^+) \gets (len, cpl)$ \;
               \Pop\;
          }
          \lElse{
               \Mark $n_x$ as \texttt{in\_route}\;     
          }
     }

     \Else{
          \Find an outgoing edge $(n_x, n_y, d_{xy})$ that is not \texttt{traversed} and $n_y$ is not \texttt{in\_route} \;
          \If {no such edge is found} {
               \Pop\;
               \Mark $n_x$ as not \texttt{in\_route}\;
               \ForEach {outgoing edge $(n_x, n_y, d_{xy})$} {
                    \Mark $(n_x,n_y, d_{xy})$ as not \texttt{traversed}\;
               }        
          }
          \nlset{22}\ElseIf{$len+ d_{xy} + \textit{sfL}[n_y] \leq \textit{fnsL}^+$ \MyAnd 
               $cpl + C(e_{wx},e_{xy},n_x) + \textit{fsC}[n_y] \leq (1\!+\!\epsilon)\!\cdot\! \textit{fsC}[n_s] $ } {
               \Push $(n_y | len+ d_{xy}, cpl + C(e_{wx},e_{xy},n_x), n_x)$\;
               \Mark $(n_x,n_y, d_{xy})$ as \texttt{traversed}\;
          }
          \lElse {
               \Mark $(n_x,n_y, d_{xy})$ as \texttt{traversed}\;
          }    
     }
}
\nlset{26}\Return $(\textit{fnsL}, \textit{fnsC}) \gets (\textit{fnsL}^+, \textit{fnsC}^+)$\;
\caption{FastestNearSimplest}
\label{algo:fastestnearsimplest}
\end{algorithm}
}

